Eccentric neutron star disk driven type II outburst pairs in Be/X-ray binaries

Be star X-ray binaries are transient systems that show two different types of outbursts. Type I outbursts occur each orbital period while type II outbursts have a period and duration that are not related to any periodicity of the binary system. Type II outbursts may be caused by mass transfer to the neutron star from a highly eccentric Be star disk. A sufficiently misaligned Be star decretion disk undergoes secular Von Zeipel-Lidov-Kozai (ZLK) oscillations of eccentricity and inclination. Observations show that in some systems the type II outbursts come in pairs with the second being of lower luminosity. We use numerical hydrodynamical simulations to explore the dynamics of the highly misaligned disk that forms around the neutron star as a consequence of mass transfer from the Be star disk. We show that the neutron star disk may also be ZLK unstable and that the eccentricity growth leads to an enhancement in the accretion rate onto the neutron star that lasts for several orbital periods, resembling a type II outburst. We suggest that in a type II outburst pair, the first outburst is caused by mass transfer from the eccentric Be star disk while the second and smaller outburst is caused by the eccentric neutron star disk. We find that the timescale between outbursts in a pair may be compatible with the observed estimates.

==> reply.tex <==
We thank the referee for providing a very useful report that significantly improved the quality of the manuscript.
We have addressed all the comments and we outline our response to each below. We have highlighted all the changes we made to the manuscript in bold text. 

Best regards,
Alessia Franchini and Rebecca Martin


===================================================

Reviewer's Comments:

The authors study the dynamics of highly misaligned disks that form around neutron stars due to mass transfer from the Be star disk. The paper presents concisely important results that shed light on the origin of type II outbursts. Nonetheless, I would like to raise several minor points:

1. The disk density profile might change due to the external interaction and deviate from the standard powerlaws. Can you please relate to the Lidov-Kozai timescale for a general powerlaw rather than -3/2 for the neutron star disk?/ relate in any other way to this issue.

R: We have modified the paper and introduced Eq. 2 that shows the global KL timescale for a generic surface density profile.

2. What is the occurrence rates of type II outbursts as derived from your model? Can you give an order of magnitude estimate and compare to the observational rates?

R: While this would certainly be a very nice and useful comparison, it is not straightforward to infer the occurrence rates of type II outburst from our calculations as these are very sensitive to the disc viscosities and temperatures that essentially regulate the mass distribution within the disc  as well as the timescale for Be star disc refilling, that we neglect. We find that the type II outbursts pair occur ~12 binary orbits apart so the prediction of the rate is different for different sources. For the sources that showed clear type II outburst pairs, we find the occurrence rate to be between 1 yr and 4 yrs depending on the specific system. 
We have added a comment on this in the conclusions section.

3. It would be interesting to mention, if possible, further specific cases that the model could explain (even for a bit different initial conditions), apart from 4U 0115+63.

R: We thank the referee for this comment. We actually found two other sources that displayed type II outbursts pairs whose occurrence can in principle be explained with our model. We added a discussion of this in Section 3.

4. An historical comment -- in the last few years it turned out that von Zeipel studied the so called 'Lidov-Kozai' oscillations back in 1916. Please add a reference to his work too.

R: Thanks for pointing this out, we have added the reference and change KL to ZLK.

